The number of clones determined by disjunctions of unary relations

We consider finitary relations (also known as crosses) that are definable via finite disjunctions of unary relations, i.e. subsets, taken from a fixed finite parameter set $\Gamma$. We prove that whenever $\Gamma$ contains at least one non-empty relation distinct from the full carrier set, there is a countably infinite number of polymorphism clones determined by relations that are disjunctively definable from $\Gamma$. Finally, we extend our result to finitely related polymorphism clones and countably infinite sets $\Gamma$.

==> hyphexcept.tex <==
%1 vim: set ft=tex:
\hyphenation{an-aly-ses}
\hyphenation{an-aly-sis}
\hyphenation{as-so-cia-tive}
\hyphenation{as-so-cia-tiv-ity}
\hyphenation{auto-morph-ic}% (2!)
%\hyphenation{auto-morph-ism}% okay
%\hyphenation{auto-morph-isms}% okay
\hyphenation{au-tono-mous}
\hyphenation{au-tono-mous-ly}% (2!)
\hyphenation{be-tween}
\hyphenation{Bool-ean}
\hyphenation{bound-ed}% (2!)
\hyphenation{Car-te-sian}
%\hyphenation{cat-egor-ies}% okay
\hyphenation{com-mu-ta-tive}
\hyphenation{com-mu-ta-tiv-ity}
\hyphenation{con-se-quence}
\hyphenation{con-se-quences}
\hyphenation{Con-se-quent-ly}% (2!)
\hyphenation{con-se-quent-ly}% (2!)
\hyphenation{co-ord-in-ate}
\hyphenation{Def-in-ition}
\hyphenation{def-in-ition}
\hyphenation{Def-in-itions}
\hyphenation{def-in-itions}
\hyphenation{de-ter-mine}
\hyphenation{de-ter-mined}
\hyphenation{de-ter-mined-ly}% (2!)
\hyphenation{de-ter-min-ing}
\hyphenation{endo-morph-ic}% (2!)
\hyphenation{endo-morph-ism}
\hyphenation{endo-morph-isms}
\hyphenation{equiva-lence}
\hyphenation{equiva-lences}
\hyphenation{equiva-lent}
\hyphenation{equiva-lent-ly}% (2!)
\hyphenation{idem-po-tent}% see po-tent
\hyphenation{idem-po-tents}
\hyphenation{iden-ti-cal}
\hyphenation{Im-pli-ca-tion}
\hyphenation{im-pli-ca-tion}
\hyphenation{Im-pli-ca-tions}
\hyphenation{im-pli-ca-tions}
\hyphenation{ir-re-du-ci-bil-ity}
%\hyphenation{ir-re-du-cible}% okay
%\hyphenation{ir-re-du-cibly}% okay
\hyphenation{iso-morph-ic} % last hyphen probably not recognised due to
%\hyphenation{iso-morph-ism}% okay
%\hyphenation{iso-morph-isms}% okay
\hyphenation{lem-ma}% (2!) % BE: not at all
\hyphenation{Lem-ma}% (2!) BE: not at all
\hyphenation{More-over}
\hyphenation{more-over}
\hyphenation{neigh-bour-hood}
\hyphenation{neigh-bour-hoods}
\hyphenation{non-au-tono-mous}
\hyphenation{poly-morph-ic}% (!2)
%\hyphenation{poly-morph-ism}% okay
%\hyphenation{poly-morph-isms}% okay
\hyphenation{posi-tive-ly}% (!2)
\hyphenation{prod-uct}
\hyphenation{prod-ucts}
\hyphenation{re-la-tion-al}% (2!)
\hyphenation{re-la-tion-al-ly}% (2!)
\hyphenation{semi-group}
\hyphenation{semi-groups}
\hyphenation{semi-lat-tice}
\hyphenation{semi-lat-tices}
\hyphenation{strength-en}% (2!)
\hyphenation{strength-ened}
\hyphenation{tauto-logic-al}% (2!)
\hyphenation{tauto-logic-al-ly}% (2!)
\hyphenation{tau-tolo-gies}
\hyphenation{tau-tolo-gous}
\hyphenation{tau-tol-ogy}
\hyphenation{topo-logic-al}% (2!)
\hyphenation{topo-logic-al-ly}% (2!)
\hyphenation{Top-olo-gies}
\hyphenation{top-olo-gies}
\hyphenation{Top-ology}
\hyphenation{top-ology}
\hyphenation{when-ever}

